Compliance for reversible client/server interactions

In the setting of session behaviours, we study an extension of the concept of compliance when a disciplined form of backtracking is present. After adding checkpoints to the syntax of session behaviours, we formalise the operational semantics via a LTS, and define a natural notion of checkpoint compliance. We then obtain a co-inductive characterisation of such compliance relation, and an axiomatic presentation that is proved to be sound and complete. As a byproduct we get a decision procedure for the new compliance, being the axiomatic system algorithmic.

==> eptcsdata.tex <==
\providecommand{\firstpage}{35}
\providecommand{\publicationstatus}{Marco Carbone (Ed.): Third Workshop on\\
Behavioural Types (BEAT 2014)\\
EPTCS 162, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.162.5}{10.4204/EPTCS.162.5}}

